A deep tree-based model for software defect prediction

Defects are common in software systems and can potentially cause various problems to software users. Different methods have been developed to quickly predict the most likely locations of defects in large code bases. Most of them focus on designing features (e.g. complexity metrics) that correlate with potentially defective code. Those approaches however do not sufficiently capture the syntax and different levels of semantics of source code, an important capability for building accurate prediction models. In this paper, we develop a novel prediction model which is capable of automatically learning features for representing source code and using them for defect prediction. Our prediction system is built upon the powerful deep learning, tree-structured Long Short Term Memory network which directly matches with the Abstract Syntax Tree representation of source code. An evaluation on two datasets, one from open source projects contributed by Samsung and the other from the public PROMISE repository, demonstrates the effectiveness of our approach for both within-project and cross-project predictions.

==> benchmarks.tex <==
\subsection{Benchmarks}

We compare the performance of our approach against the following benchmarks:

\textbf{Software metrics}:  Complexity metrics have been extensively used for defect prediction (e.g. \cite{Hall:2012}) and vulnerability prediction (e.g. \cite{Shin:2011:ECC,Shin:2008:EMP,Chowdhury:2011:UCC}). This is resulted from the intuition that complex code is difficult to understand, maintain and test, and thus has a higher chance of having vulnerabilities than simple code. We have implemented a vulnerability prediction models based on 60 metrics. These features are commonly used in existing vulnerability prediction models. They covers 7 categories:  cohesion metrics, complexity metrics, coupling metrics, documentation metrics, inheritance metrics, code duplication metrics, and size metrics.


\textbf{Bag of Words}: This technique has been used in previous work \cite{ScandariatoWHJ14}, which also consider source code as a special form of text. Hence, it treats a source file as a collection of terms associated with frequencies. The term frequencies are the features which are used as the predictors for a vulnerability prediction model. Lexical analysis is done to source code to break it into a vector of code tokens and the frequency of each token in the file is counted. We also followed previous work \cite{ScandariatoWHJ14} by discretizing the BoW features since they found that this method significantly improved the performance of the vulnerability prediction models. The discretization process involves transforming the numerical BoW features into two \emph{bins}. If a code token occurs more than a certain threshold (e.g. 5 times) than it is mapped to one bin, otherwise it is mapped to another bin.


\textbf{Deep Belief Network}: Recent work \cite{Wang:2016:ALS} has demonstrated that Deep Belief Network (DBN) \cite{hinton2006rdd} worked well for defect prediction. DBN is a family of stochastic deep neural networks which extract multiple layers of data representation. In our implementation, DBN takes the word counts per file as input and produces a latent posterior as output, which is then used as a new file representation. Since the standard DBN accepts only input in the range [0,1], we normalize the word counts by dividing each dimension to its maximum value accross the entire training data. The DBN is then built in a stage-wise fashion as follows. At the bottom layer, a Restricted Boltzmann Machine (RBM) is trained on the normalized word count. An RBM is a special two-layer neural network with binary neurons. %Unlike the standard neural networks, which learn a mapping from an input to an output in an supervised manner, RBM learns a distribution of data using unsupervised learning (i.e., without labels).
Following the standard practice in the literature, the RBM is trained using Contrastive Divergence \cite{hinton2006rdd}. After the first RBM is trained, its posterior is used as the input for the next RBM, and the training is repeated. Finally, the two RBMs are stacked on top of each other to form a DBN with two hidden layers. The posterior of the second RBM is used as the new file representation. In our implementation, the two hidden layers have the size of 500 and 128, respectively.

To enable a fair comparison, we used the same classifier for our prediction models and all the benchmarks. We chose Random Forests (RF), an ensemble method which combines the estimates from multiple estimators since it is one of the most effective classifier for vulnerability prediction \cite{ScandariatoWHJ14}. We employed the standard Precision, Recall, and F-measure, which has been widely-used in the literature (e.g. \cite{ScandariatoWHJ14,Shin:2011:ECC,Chowdhury:2011:UCC,Zimmermann:2010:SNH}) for evaluating the predictive performance of vulnerability prediction models built using the three above benchmarks and our approach.



==> introBackground.tex <==


\section{Background}
\subsection{Recurrent Neural Network with Long Short Term Memory Units}
%Weight matrices within a neural network, randomized at the start are adjusted based on the produced output and the expected output.

Recurrent neural networks takes in an order-sensitive sequential input \textbf{w} (e.g \ref{fig:lstm}), usually in the form of vectors, processed by the neural network which could be made up of different number of layers, and produces an output \textbf{s}, once again in the form of a vector. For example, if an input is in the form of language text, it can converted into vectors using different state-of-the-art techniques [cite somethings]. Let $w_{1},\ldots,w_{n}$ be a sequence of code, used as input, and $y_{1},\ldots,y_{n}$, the corresponding labels, as the expected output. The produced output at the previous time step \textit{t - 1} is used as one of the input for the current time step \textit{t} neural network. The output of the current time step $s_t$ is computed using the formula below.

\begin{equation}
	s_{t} = \sigma (\textbf{b} + W_{tran}s_{t-1} + W_{in}w_{t})
\end{equation}

where $\sigma$ is a nonlinear element-wise transform function while \textbf{b}, $W_{tran}$ and $W_{in}$ are referred as model parameters. Sharing the same set of parameters allows training of the RNN model with lesser number of samples as compared to not sharing any parameters. The error between the expected output and the predicted output are passed backwards through the network to allow adjustment of the model parameters during the training phase. This in return minimizes the error. Values of the input vectors are also adjusted accordingly.

RNNs has been used to solve a variety of problems, for example speech recognition, language modeling and image captioning. However, recurrent neural networks are only capable of capturing context within short distances. Recurrent Neural Networks with Long Short-Term Memory units overcomes this shortcoming by introducing a \textit{memory cell}, \textit{$c_t$}. The memory cells makes it possible to capture long term dependencies by determining how much information will be relevant in predicting the next sequence. The amount of information flowing through the memory cell is controlled by three different gates, namely the input gate, the forget gate and the output gate. An example of RNN with LSTM is shown in \ref{fig:lstm_unit}.

\subsection{Tree-Structured LSTMs}

Tree LSTM allows learning to be done in the form of a syntax tree, unlike traditional LSTM which is strictly used with sequential data. Traditional LSTM can be seen as a form of  tree-structured LSTM with each node having only 1 child.  Tree-LSTM takes in input from all existing child nodes for the prediction of the current node instead of just the output from the previous input in traditional LSTM. Tree LSTM selectively learns relevant information by utilizing forget gates of every child nodes. An example of a short code segment broken down into an Abstract Syntax Tree using JavaParser \footnote{https://github.com/javaparser/javaparser} is shown in \ref{fig:lstm_unit}. Tree-LSTM can be broken down into two different types, the \textit{Child-Sum Tree-LSTM} and the \textit{N-ary Tree-LSTM}.

\subsubsection{Child-Sum Tree-LSTM}
In the Child-Sum Tree-LSTM we can interpret the parameter matrix used in the neural network as encoding the correlations between the input and the hidden states of the child nodes. The components within the Child-Sum Tree LSTM is made up of the sum of child hidden states making it suitable for trees with high branching factors or unordered child nodes. A Child-Sum Tree LSTM applied to a dependency tree is referred as a Dependency Tree-LSTM. In a dependency tree, the number of child nodes a particular node depends on is highly variable.

\subsubsection{N-ary Tree-LSTM}
The branching factor in a N-ary Tree-LSTM is at most N. The child nodes must be ordered, the child nodes are indexed from 1 to N. Different parameter matrices are used for each child nodes allowing the model to be learn more fine-grained conditioning on the state of the child nodes as compared to Child-Sum Tree-LSTM. \textbf{Parameterization} is done on the forget gate of certain child nodes to allow more flexible control of information from child to parent nodes. If the branching factor is large, it becomes impractical to use the additional parameters and it is set to having the same values or 0.

Binary Tree-LSTM units can be applied to inarized constituency trees since the left and right child nodes are distinguished. This is referred as \textit{Constituency Tree-LSTM`}.

\begin{figure}
	\label{fig:lstm}
	\includegraphics[width=8cm]{figures/lstm.png}
	\caption{A recurrent neural network.}
\end{figure}

\begin{figure}
	\label{fig:lstm_unit}
	\includegraphics[width=8cm]{figures/lstm_unit.png}
	\caption{The internal structure of a Neural Network with Long Short-Term units}
\end{figure}

\begin{figure}
	\label{fig:ast}
	\includegraphics[width=8cm]{figures/AST_example.png}
	\caption{Code example "int i = 0;" broken down into an Abstract Syntax Tree}
\end{figure}

\cite{Ablamowicz07}


%\begin{figure}
%\includegraphics[width=8cm]{images/lstm2.png}
%\caption{A sample black and white graphic.}
%\end{figure}




==> motivation.tex <==
\section{Motivation}

\setbox0=\hbox{%
\begin{minipage}{1.5in}
\begin{lstlisting}[caption=File1.java]
int a = 10;
int count = 100;
int MAX = maxInt();
for(int i = 0; i 
 < count; i++){
   if(a += count 
    < MAX){
 	 a++;
   }
}
\end{lstlisting}
\end{minipage}
}
\savestack{\listingA}{\box0}

\setbox0=\hbox{%
\begin{minipage}{1.5in}
\begin{lstlisting}[caption=File2.java]
int a = 10;
int count = 100;
int MAX = maxInt();
if(a += count 
 < MAX){
   for(int i = 0; i 
	< count; i++){
	 a++;
   }
}
\end{lstlisting}
\end{minipage}
}
\savestack{\listingB}{\box0}


\begin{figure}[ht]
    \begin{tabular}{|c|c}
    \listingA &
    \listingB \\
    \end{tabular}
    \caption{A motivating example}
	\label{fig:example}
\end{figure}
